Can Language Models Enable In-Context Database?

Large language models (LLMs) are emerging as few-shot learners capable of handling a variety of tasks, including comprehension, planning, reasoning, question answering, arithmetic calculations, and more. At the core of these capabilities is LLMs' proficiency in representing and understanding structural or semi-structural data, such as tables and graphs. Numerous studies have demonstrated that reasoning on tabular data or graphs is not only feasible for LLMs but also gives a promising research direction which treats these data as in-context data. The lightweight and human readable characteristics of in-context database can potentially make it an alternative for the traditional database in typical RAG (Retrieval Augmented Generation) settings. However, almost all current work focuses on static in-context data, which does not allow dynamic update. In this paper, to enable dynamic database update, delta encoding of database is proposed. We explore how data stored in traditional RDBMS can be encoded as in-context text and evaluate LLMs' proficiency for CRUD (Create, Read, Update and Delete) operations on in-context databases. A benchmark named InConDB is presented and extensive experiments are conducted to show the performance of different language models in enabling in-context database by varying the database encoding method, prompting method, operation type and input data distribution, revealing both the proficiency and limitations.

==> preliminary.tex <==
\section{Preliminaries}
\label{sec:preliminary}
Here we give the basic definitions and terminologies necessary to the descriptions in the following sections. We also give the key observation which helps to form the intuitive idea of our work.

\subsection{Definitions}

\inlinesubsection{Definition 1 Object Set.}An Object Set $O=\{O[1],...,O[n]\}$ is a set of $n$ objects, in which $i$th object can be written as $O[i]=(V[i],M_1[i],...,M_k[i])$. Here $V$ is the list of vectors and $M_j,j\in [1,k]$ is the $j$th list of meta-data, which can be either attributes (discrete values) or scalar values. So the Object Set can also be written as a tuple: $O=(V,M_1,...,M_k)$. 

\inlinesubsection{Definition 2 Filtering Constraint.}A Filtering Constraint $c$ is a predicate, which is a boolean function defined on $\{M_1,...,M_k\}$. $O(c)$ is the filtered subset of $O$ which satisfy $c$, that is, $O(c)=\{O[i]\ |\ c(O[i])=True\}$. For instance, $O(c) = \{O[i]\ |\ M_1[i]=m_1 \cap M_2[i]=m_2\ \cap ,...,\cap\ M_k[i] \in [m_k^{lower},m_k^{upper}]\}$. Here $c$ is a combination of attributes and range filters.

If constraint $O(c_1) \subseteq O(c_2)$, then $c_1$ is called the sub-constraint of $c_2$, indicating it's more strict than $c_2$ and $c_2$ is called the super-constraint of $c_1$.

\inlinesubsection{Definition 3 Constraint Space.} A constraint space $C$ is the set of filter constraints. The constraint space $C$ can usually be parameterized into a multi-dimensional space and the way of parametrization depends on specific constraint types and requirements of the applications. For instance, for $c$ in Def. 2, we can represent if with $(m1,m2,...,m_k^{lower},m_k^{upper})$.

\inlinesubsection{Definition 4 Metrics}

\inlinesubsection{Definition 4 Hybrid Query(HQ).}A Hybrid Query is a tuple $q=(c,v)$, in which $c$ is a constraint and $v$ is a $D$-dimensional vector. We want to find the set $T$ of $k_V$ objects in the Object Sets $O$ which minimize $\sum_{i\in T} d(V[i],v)$ w.r.t some distance metric $d$, such that $\forall i \in T, c(O[i])=True$. Formally, we need to retrieve the set:
\begin{align*}
T&=\argmin_{|T|=k_V} \sum_{i\in T} d(V[i],v)\\
  &s.t\ \forall i\in T, O[i] \in O(c)
\end{align*}
To facilitate search on Object Set $O=\{O[1],...,O[n]\}$, indexes of various types can be built on $O$. 

\inlinesubsection{Definition 5 Tree based Indexes.} Here on constraint space $C$, we can define a tree based index as $T_C=(C,E_C)$, in which $E_C$ is the set of directed links from parent constraint to children constraint. If $(C[i],C[j]) \in E_C$, then $O(C[i]) \subset O(C[j])$, that is, the child constraint is always more strict than the parent constraint. Also for the root node $r_C$ of $T_C$, we have $O(r_C) = O$. Minimal Super-Constraint Search will be conducted on $T_C$, which we'll introduce in detail in \ref{sec:framework}.

\inlinesubsection{Definition 6 Graph based Indexes.}As the typical graph-based ANNS indexes, we can build an index $G_V=(V,E_V)$ on the vector set $V$, where $E_V$ is the directed edges among $V$. $G_V$ is normally a variant of some types of base graphs, such as Delaunay Graph, Relative Neighborhood Graph, K-Nearest Neighbour Graph and Minimum Spanning Tree\cite{}. Best First Search (BFS) and its variant is the search (routing) algorithm on $G_V$, which we'll introduce more in \ref{sec:framework}.

%\inlinesubsection{Definition 7 Best First Search} 
\subsection{Filtering Patterns}
\label{subsec:filtering_patterns}
From the first look, Hybrid Query is much different than pure ANNS, however there are some key observations we can utilize to reduce HQ to ANNS with minimal overhead.

\inlinesubsection{Definition 7 Constraint-Induced Subgraph.}Suppose we've built a graph-based ANNS indexes $G_V$ on $V$. Now for the filtering constraint $c$, we can get a subgraph $G_V(c)=(V(c),E_V(c))$, where $V(c)$ corresponds to $O(c)$ and $E_V(c)$ is the set of all the edges with both endpoints in $V(c)$. $G_V(c)$ is called the subgraph of $G_V$ induced by the constraint $c$. 

It is easily to observe that $G_V(c)$ itself may not be connected, and as a result suppose it contains $m$ connected components. We can put each of the connected components as $G_V^i(c)$ and thus $G_V(c)=\{G_V^i(c)|\ \forall i \in [1,m],\ G_V^i(c) \subset G_V\}$. For each of the connected components, there is a representative node which has a path to all of the nodes within the connected component, we can put the set of all the representative node as $V_p(c)$.



\inlinesubsection{Observation 1 Distribution of Filtered Subset $O(c)$}


\inlinesubsection{Observation 2 Connected Components on $G_V$.}
According to the percolation theory\cite{}, as the cardinality $|O(c)|$ increases (namely $c$ becomes less strict), the average size of each connected component will increase, until reaching a point where all the nodes in $G_V(c)$ are connected. Similarly towards the other extreme, as $|O(c)|$ decreases ($c$ becomes more strict), the average size of each connected component will decrease, until $c$ becomes too strict that $O(c) = \emptyset$. So for every $C$ and $G_V$, there has to be an upperbound for the number of connected components in $G_V(c)$. Figure \ref{} illustrates the number of connected components as a function of the cardinality $|O(c)|$.
